DeepGate2: Functionality-Aware Circuit Representation Learning

Circuit representation learning aims to obtain neural representations of circuit elements and has emerged as a promising research direction that can be applied to various EDA and logic reasoning tasks. Existing solutions, such as DeepGate, have the potential to embed both circuit structural information and functional behavior. However, their capabilities are limited due to weak supervision or flawed model design, resulting in unsatisfactory performance in downstream tasks. In this paper, we introduce DeepGate2, a novel functionality-aware learning framework that significantly improves upon the original DeepGate solution in terms of both learning effectiveness and efficiency. Our approach involves using pairwise truth table differences between sampled logic gates as training supervision, along with a well-designed and scalable loss function that explicitly considers circuit functionality. Additionally, we consider inherent circuit characteristics and design an efficient one-round graph neural network (GNN), resulting in an order of magnitude faster learning speed than the original DeepGate solution. Experimental results demonstrate significant improvements in two practical downstream tasks: logic synthesis and Boolean satisfiability solving. The code is available at https://github.com/cure-lab/DeepGate2

==> 01_into_bak.tex <==
\section{Introduction}
% Deep learning has been widely applied in various fields and has recently sparked a trend of using it to assist in Electronic Design Automation (EDA), such as routing~\cite{chen2020pros, mirhoseini2021graph}, synthesis~\cite{neto2019lsoracle, haaswijk2018deep}, and testing~\cite{shi2022deeptpi, huang2022neural}. Most previous works model circuits as graphs, with logic gates as nodes and wires as edges~\cite{mirhoseini2021graph, shi2022deeptpi, ma2019high, li2022deepgate, wang2022functionality, lopera2021survey}. As a result, an intuitive and widely used approach to analyze the graph is applying Graph Neural Networks (GNNs) to learn circuit representations and handle downstream tasks.

% Deep learning has been widely applied in various fields and has recently sparked a trend of being used %using it
% to assist in Electronic Design Automation (EDA), such as routing~\cite{chen2020pros, mirhoseini2021graph}, synthesis~\cite{neto2019lsoracle, haaswijk2018deep}, and testing~\cite{shi2022deeptpi, huang2022neural}.

The recent trend of applying Deep Learning (DL) techniques in Electronic Design Automation (EDA) fields has boosted the tools for various tasks, such as routing~\cite{chen2020pros, mirhoseini2021graph}, synthesis~\cite{neto2019lsoracle, haaswijk2018deep}, and testing~\cite{shi2022deeptpi, huang2022neural}.
Among the existing learning-based EDA solutions, the circuit representation learning paradigm~\cite{li2022deepgate, wang2022functionality, zhu2022tag, lai2022maskplace} has emerged as a promising research direction. Instead of training standalone models for each EDA task from scratch, this paradigm represents the circuits into embedding vectors, which are further applied for various downstream tasks. 

% 问题：GNN过分关注结构，而非功能
% Although powerful, GNNs tend to focus excessively on the topological structure of graphs, instead of functionality~\cite{fayyazi2019deep, he2021graph}. For instance, when two circuits differ only in one logic gate type, GNNs may still produce similar representations, even if the functionality changes dramatically. In fact, the logical functionality rather than the structure is one of the most crucial aspects of circuit analysis in design phase. For example, logic synthesis tools parse the netlist to obtain the nodes' functionality, then merge nodes with similar~\cite{sawada1995logic} or equivalent~\cite{kuehlmann2004dynamic} functional behaviors. 
% Although powerful, GNNs tend to focus on the topological structure of graphs, but overlook the underlaying semantic, i.e., circuit functionality. For example, if two circuits differ only in one logic gate type, GNNs may still produce similar representations, even if the functionality changes dramatically~\cite{fayyazi2019deep, he2021graph}. In fact, functionality is one of the most crucial aspects of many EDA tasks, such as logic synthesis~\cite{kuehlmann2004dynamic, sawada1995logic}. 

Existing circuit representation learning models, such as~\cite{li2022deepgate, wang2022functionality, zhu2022tag, fayyazi2019deep, he2021graph}, formulate circuits as graphs and use the graph neural networks (GNNs) to model circuit. Some of them~\cite{zhu2022tag, fayyazi2019deep, he2021graph} consider the gate connections to capture the structural information of circuits. For example, \cite{he2021graph} learns analog and mixed-signal circuit representation from the circuit netlist with layout position. \cite{he2021graph} employs a customized GNN to learn circuit structure and predict module boundaries. 

While these structure-based models have shown promising results in a few applications, they ignore the underlying functionality of circuits, i.e., the logic behaviour, and lack of the ability to generalize to other tasks. For instance, these models are not competent of improving logic synthesis tools, which simplify circuits by merging gates with similar~\cite{sawada1995logic} or equivalent~\cite{kuehlmann2004dynamic} functional behaviors. Therefore, a good circuit representation should encode the circuit structure along with its functionality. 


% Although powerful, GNNs tend to focus on the topological structure of circuits and ignore their underlying functionality, i.e., the logic behaviour. For example, if two circuits differ only in one logic gate type, GNNs may still produce similar representations, even if their %behaviour change dramatically
% underlying functionality is quite different~\cite{fayyazi2019deep, he2021graph}.
% Logic functionality is perhaps one of the most important components of circuit analysis.
% %In fact, logical functionality is one of the most crucial aspects of circuit analysis. 
% For example, logic synthesis tools parse the circuit to obtain the gates' functionality, then merge gates with similar~\cite{sawada1995logic} or equivalent~\cite{kuehlmann2004dynamic} functional behaviors. Therefore, a good circuit representation should encode the underlying circuit functionality along with its structure.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Motivation：GNN层数多，oversmooth
%首先，目前的方法缺乏与电路功能相关的有效监督。电路节点功能最直接的体现是真值表，获得完整的真值表需要消耗大量时间进行完备仿真，同时真值表长度不定，受电路primary inputs (PI)数量决定，因此模型学习预测真值表是个不太可能完成的任务。[XX]认为随机仿真下门为logic-1的概率可以作为与电路功能有关的监督，一种直观的解释是真值表中logic-1的占比。很显然，logic probability为0.5的逻辑非门的fan-in gates的logic prbability也是0.5，但二者真值表完全颠倒。[XX]使用对比学习来训练模型区分功能等价电路和功能不等价电路。但这种方法需要靠扰动原是电路生成功能不等价电路，当扰动较小时，训练好的模型很难发现两个结构天差地别但功能一致的电路。

%其次，目前电路学习模型的建模能力不足。由于重汇聚结构的存在，电路中两个节点的逻辑功能并非完全独立，我们不可能仅仅通过某个2-inputs逻辑门的两个fan-in门的功能推导出该门的功能，必须要考虑二者的扇入结构。因此获得电路完备的逻辑功能也就成为了NP-hard问题。同样，GNN的主要操作是邻居节点之间互相message-passing，因此GNN也就无法通过单次forward propagation学习某一门的逻辑功能。传统的做法是增加GNN传播轮数[XX]或执行双向传播[XX]来捕获门之间的结构相关性。但随着节点之间信息传播次数增加，图中节点的embedding会趋同，也就是会出现over-smooth现象[XX]，对寻找电路节点间的差异性起到了负面作用。

% On the one hand, the previous circuit learning frameworks lack effective supervision related to circuit functionality. While a circuit's truth table is the most direct representation of its gate functionality, obtaining a complete truth table through exhaustive simulation is impractical due to the time requirements, which increases exponentially with the number of primary inputs (PIs). As an alternative, \cite{li2022deepgate} suggests that the probability of logic-1 under random simulation can be treated as a functional supervision, which is the proportion of logic-1 in the truth table. However, a counterexample is that a NOT gate with $0.5$ logic-1 probability has a fan-in gate also with $0.5$ logic-1 probability, yet their truth tables are completely inverted. Besides, \cite{wang2022functionality} applies contrastive learning to distinguish between functionally equivalent and inequivalent circuits. However, such self-supervised manner relies on circuit transformation to generate dataset and ignores the supervision signal within the circuit, resulting in low data efficiency. 

% Although existing circuit representation learning frameworks~\cite{li2022deepgate, wang2022functionality} attempt to capture the logic functionality, they suffers from two major shortcomings. %there are still two existing shortcomings.
The others circuit representation learning models~\cite{li2022deepgate, wang2022functionality} attempt to capture the logic functionality, but they suffers from two major shortcomings. 
On the one hand, these solutions %existing circuit learning frameworks 
lack effective supervision related to circuit functionality. For example, \cite{wang2022functionality} learns to distinguish between functionally equivalent and inequivalent circuits by contrastive learning. However, such self-supervised manner relies on a weak supervision by circuit augmentation. In fact, circuit truth table is the most direct representation of functionality. Unfortunately, obtaining a complete truth table through exhaustive simulation is impractical due to the time requirements, which increases exponentially with the number of primary inputs (PIs). DeepGate~\cite{li2022deepgate} suggests that the probability of logic-1 in the incomplete truth table can be treated as a functional supervision and simulates circuits within acceptable time to prepare such labels. However, a counterexample is that a NOT gate with $0.5$ logic-1 probability has a fan-in gate also with $0.5$ logic-1 probability, yet their truth tables are completely inverted. 


%\cite{wang2022functionality} applies contrastive learning to distinguish between functionally equivalent and inequivalent circuits. However, the self-supervised manner ignores the the inherent properties of the circuit, such as truth table. this approach relies on perturbing the original circuit to generate functionally equivalent circuits. When the perturbation is not heavy, it is challenging for the trained model to identify circuits with vastly different structures but identical functionality.

% Another limitation of current circuit learning models is their insufficient modeling capability. Due to the presence of reconvergence structures, the behaviors of two nodes are not entirely independent. Deducing the function of a 2-input logic gate solely based on the behaviors of its two fan-in gates without considering their predecessors is not possible. Obtaining the complete logical functionality is an NP-hard problem~\cite{krishnamurthy1987dynamic}. Similarly, the fundamental operation of GNN is message-passing between neighboring nodes. Thus, GNN still cannot learn the functional information of a certain gate through a single forward propagation. Traditional approaches include increasing the number of GNN propagation rounds~\cite{wu2023gamora, ma2019high} or performing bidirectional propagation~\cite{li2022deepgate} to capture the structural correlations between gates. However, as the number of message-passing rounds increases, the node embeddings become more similar, leading to over-smoothing~\cite{li2018deeper}, that adversely affects the ability to differentiate gate functionality based on the embeddings. 

On the other hand, previous circuit learning models consider the inherent characteristics of circuits insufficiently. Specifically, the functionality of each PI is independently and identically distributed, meaning that the logic value of each PI is not affected by others, and the logic probability of each PI is equal. Most of the existing circuit learning models~\cite{wu2023gamora, ma2019high, li2022deepgate, wang2022functionality} simply assign the same initial embedding to all PIs to mimic the identical distribution of PI behaviours. However, these models lack unique identifications for PIs and ignore to consider the PI independence in model design. As a result, to capture circuit features, these models must discover the graphic canonical identifications by multiple rounds of message-passing, which is time-consuming and impractical for modern industrial circuits.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Our method：
% 第二，我们设计了一种one-round GNN来快速建模电路结构与功能信息。我们的GNN区分node functional embedding 和 structural embedding，在更新structrual embedding时只需要聚合每个节点前驱的信息，而在更新functional embedding时需要考虑前驱的functional information和前驱节点的结构相关性，也就是是否存在重汇聚结构。为了训练这样的网络，我们为PI的初始embedding赋值互相正交的向量，他们在embedding space上均独一无二且互相距离相等，也就是说PI有了独一无二的身份编码。这样做的目的能够直观的解释为，通过记录两个节点是否有一个或多个共同的PIs来判断他们是否存在结构相关性。这种GNN能够只通过one round前向message-passing来学习电路的结构和功能信息，避免了over-smooth现象，并提高了模型推理效率。

% Firstly, our model predicts the functional similarity between node pairs within the same circuit. More specifically, we design a functionality-aware loss function to minimize the error between pairwise truth table hamming distance and node embedding distance. The node embedding distance can be calculated based on the cosine similarity of two node embedding vectors. Compared to the previous work, our approach provides more rich supervision related to functionality and avoid the performance limitation caused by data generation. 
% These vectors are unique and equidistant in the embedding space, which means each PI has a unique positional encoding. An intuitive explanation should be that the purpose is to determine whether two nodes are reconvergent by recording whether they share one or multiple common PIs. Our GNN learns both the structural and functional information through only one round forward message-passing, avoiding embedding over-smoothing and improving the efficiency.

Therefore, \textit{functionality-aware circuit representation learning} is a remaining challenge. To address this challenging problem, in this paper we propose a \textit{Functionality-aware Circuit Learning Framework}. Firstly, we use the pairwise truth table difference as supervision because it is highly related to functionality and is easily obtained. To be specific, we design a functionality-aware loss function to minimize the error between pairwise node embedding distance in embedding space (prediction) and the Hamming distance of truth table (ground truth). More importantly, our approach does not require the complete simulation to prepare ground truth and supports training with incomplete truth tables. Consequently, compared to the previous inefficient supervision, the proposed supervision embeds the genuine functional information and can be scaled to large circuits. 

Secondly, we design a one-round graph neural network (GNN) to efficiently model both structural and functional features of each logic gate. Our GNN separates the node functional embedding and structural embedding, and is equipped with an initialization strategy. During structural embedding updating, GNN only aggregates the structural embeddings from the predecessors. During functional embedding updating, GNN considers both the functional information and the structural correlation of the predecessors, analogizing the traditional circuit analysis approaches~\cite{ockunzzi2001breaking, gu1991testability}. At the beginning of model training, we assign orthogonal vectors as the initial embeddings for PIs. These vectors are unique and equidistant each other in the embedding space, mimicking the independently and identically distributed PI behaviour, respectively. With the above strategies, our model can capture both the structural and functional information through a single round forward message-passing, which is more efficient than previous methods.

 
% [4.18 删] Firstly, our model does not attempt to differentiate whether two circuits are functionally equivalent, but rather predicts the similarity of functionality between two nodes within the same circuit. More specifically, we use truth tables containing functional information to supervise the functionality-aware training, with the goal of minimizing the difference between the similarity of node embedding pairs and the similarity of the truth table pairs. Compared to the contrastive learning approach~\cite{wang2022functionality}, this method provides more rich supervision and avoid much time on sample pairs generation. 

% [4.18 删] Secondly, the functionality of each multi-fan-in gate is related to the correlations between its input gates and the reason for correlations is fundamentally due to the presence of reconvergent fan-in structures. Although methods~\cite{chen2019testability, gu1991testability} attempt to compensate for the effects of reconvergence on circuit functionality analysis by increasing node correlations as a correction term, identifying complete reconvergence information is an NP-hard problem~\cite{krishnamurthy1987dynamic}. Previous GNNs could only encode local circuit structures as completely as possible through multiple rounds of forward and backward message passing, and even required special structures to handle reconvergence (such as skip connections). We believe that a necessary condition for the reconvergence is that the node pair shares a common primary input (PI). In our method, we assign a \textit{unique identification} to each primary input. During the process of forward message passing, when two nodes have PI overlapping, their embeddings will have a higher degree of similarity. The PI "position encoding" strategy avoids the demand for multiple iterations of message-passing.

Thirdly, we investigate the effectiveness of our proposed functionality-aware circuit learning framework on two real-world applications: logic synthesis~\cite{mishchenko2005fraigs} and Boolean satisfiability (SAT) solving~\cite{queue2019cadical}. The model informs the logic synthesis tool which nodes have higher functional similarity, thereby reducing the search space for the synthesis tool. Additionally, during the branching process of SAT solving, we make the same branching decisions for nodes with similar functionality as the current branching node. The experimental results indicate that our framework benefits downstream applications that rely on circuit functionality. 


The contributions of this paper are summarized as follows:
\begin{itemize}
    \item We supervise the model training with pairwise truth table difference and design a novel functionality-aware loss function. Our strategies involve a strong supervision related to functionality and are able to scale to large circuit. 
    \item We involve the circuit inherent characteristics into model design and purpose a one-round GNN model. The model learn both structural and functional information separately, and includes an embedding initialization strategy. Our model can obtain rich circuit representation only with one round of message-passing operation. 
    \item We apply the model to two downstream applications: logic synthesize and SAT solving. The experimental results show that our model can accelerate the existing tools on these tasks. 
\end{itemize}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Roadmap 
% xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx xx 

==> bak_exp.tex <==
\section{Experiments}
\subsection{Experiment Settings}
\subsubsection{Dataset Preparation}
We use the circuits in DeepGate-v1~\cite{li2022deepgate}, which are extracted from ITC’99~\cite{ITC99}, IWLS’05~\cite{albrecht2005iwls}, EPFL~\cite{EPFLBenchmarks} and OpenCore~\cite{takeda2008opencore}. These circuits consists of $10,824$ AIGs with sizes ranging from $36$ to $3,214$ logic gates. To obtain the incomplete truth table, we set the number of simulation patterns is $15,000$. Based on the data preparation method described in Section.~\ref{Sec:Method:Data}, the resulting dataset contains $894,151$ node pairs. We create 80/20 training/test splits for model training and evaluation. 

\subsubsection{Evaluation Metrics} \label{Sec:Exp:Acc}
We assess our DeepGate-v2 with two tasks. The first task is to predict the logic probability for each logic gate. We calculate the average prediction error (PE) as Eq.~\eqref{Eq:AccTask0Prob}, where the set $\mathcal{V}$ includes all logic gates. 
\begin{equation} \label{Eq:AccTask0Prob}
    PE = \frac{1}{|\mathcal{V}|} \sum_{i \in \mathcal{V}}|P_i - \hat{P}_i|
\end{equation}


The second task is to identify the logic equivalent gates within a circuit. A gate pair $(i, j)$ is considered as a positive pair if these two logic gates $i$ and $j$ have the same function, where the pairwise Hamming distance of truth tables $D_{(i, j)}^T = 0$. If the similarity $S_{(i, j)}$ between these two embedding vectors $hf_i$ and $hf_j$ exceeds a certain threshold, the model will recognize the gate pair $(i, j)$ as equivalent. The optimal threshold $\theta$ is determined based on the receiver operating characteristic (ROC). The evaluation metrics is formally defined in Eq.~\eqref{Eq:AccTask1}, where $TP$, $TN$, $FP$, $FN$ are true positive, true negative, false positive and false negative, respective, and $M$ is the total number of gate pairs. In the following experiments, the performance on logic equivalent gates identification is measured in terms of \text{Recall}, \text{Precision}, \text{F1-Score} and area under curve (AUC). 
\begin{equation} \label{Eq:AccTask1}
    \begin{split}
        TP & = \frac{\sum( (D_{(i, j)}^T == 0) \ \& \ (S_{(i, j)} > \theta))}{M} \\
        TN & = \frac{\sum( (D_{(i, j)}^T > 0) \ \& \ (S_{(i, j)} < \theta))}{M} \\
        FP & = \frac{\sum( (D_{(i, j)}^T > 0) \ \& \ (S_{(i, j)} > \theta))}{M} \\
        FN & = \frac{\sum( (D_{(i, j)}^T == 0) \ \& \ (S_{(i, j)} < \theta))}{M} \\
        % Recall & = \frac{TP}{TP + FN} \\ 
        % Precision & = \frac{TP}{TP + FP} \\ 
        % F1-Score & = \frac{2 * TP}{2 * TP + FP + FN} \\ 
    \end{split}
\end{equation}

% 我们采样两对gates (i, j) and (p, q)，其中一对真值表的汉明距离D_{(i, j)}^T小于D_{(p, q)}^T，如果模型得到的embedding的距离也满足D_{(i, j)}^H小于D_{(p, q)}^H，我们认为这是一次成功的采样。我们定义模型精度为：100次采样中，成功采样的占比。
The second task involves predicting the functional similarity. To be specific, we sample two pairs of gates $(i, j)$ and $(p, q)$, where one pairwise Hamming distance of truth tables $D_{(i, j)}^T$ is less than that of $D_{(p, q)}^T$. If the distance of the embedding defined in Eq.~\eqref{Eq:Cos} also satisfies that $D_{(i, j)}^H$ is less than $D_{(p, q)}^H$, we consider this a successful sampling. We define the accuracy $ACC$ as the proportion of successful samplings out of $K$ attempts in~\eqref{Eq:AccTask2}. In our experiments, we set $K=10,000$
\begin{equation} \label{Eq:AccTask2}
    ACC = \frac{\sum ((D_{(i, j)}^T < D_{(p, q)}^T) \& (D_{(i, j)}^H < D_{(p, q)}^H))}{K}
\end{equation}

We conduct the following performance comparisons on $10$ industrial circuits, with circuit sizes ranging from $3.18k$ gates to $40.50k$ gates. The circuit characters are listed in Table.~\ref{TAB:Comp:Task1} and Table.~\ref{TAB:Comp:Task2}. 

\subsubsection{Model Settings}
In the one-round GNN model configuration, the dimension of both structural embedding $hs$ and functional embedding $hf$ is $64$. Both $MLP_{prob}$ and $MLP_{rc}$ contain $1$ hidden layer with $32$ neurons and a ReLu activation function. During model training, we use the ADAM optimizer with the learning rate $0.0001$ and train for $60$ epochs to ensure each model can converge. The other models~\cite{li2022deepgate, wang2022functionality} mentioned in the following experiments maintain their original settings and are trained until they converge. 

\subsection{Comparison with other Models}
This section compares the functionality-aware accuracy defined in Section.~\ref{Sec:Exp:Acc} with another two circuit learning models~\cite{li2022deepgate, wang2022functionality}. The DeepGate~\cite{li2022deepgate} model treats the logic probability as supervision since it contains the statistical information of truth table. The FGNN~\cite{wang2022functionality} is trained to differentiate between logic equivalent and inequivalent circuits using contrastive learning. 

% Task 1
\begin{table*}[!t]
\centering
\caption{Performance of Different Models on Logic Equivalent Gates Identification} \label{TAB:Comp:Task1}
\renewcommand\tabcolsep{4.0pt}
\begin{tabular}{@{}ll|llll|llll|llll@{}}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{Circuit}} & \multicolumn{1}{c|}{\multirow{2}{*}{Size}} & \multicolumn{4}{c|}{Our}                                                                                             & \multicolumn{4}{c|}{DeepGate~\cite{li2022deepgate}}                                                                                        & \multicolumn{4}{c}{FGNN~\cite{wang2022functionality}}                                                                                            \\
\multicolumn{1}{c}{}                         & \multicolumn{1}{c|}{}                      & \multicolumn{1}{c}{Recall} & \multicolumn{1}{c}{Precision} & \multicolumn{1}{c}{F1-Score} & \multicolumn{1}{c|}{AUC} & \multicolumn{1}{c}{Recall} & \multicolumn{1}{c}{Precision} & \multicolumn{1}{c}{F1-Score} & \multicolumn{1}{c|}{AUC} & \multicolumn{1}{c}{Recall} & \multicolumn{1}{c}{Precision} & \multicolumn{1}{c}{F1-Score} & \multicolumn{1}{c}{AUC} \\ \midrule
D1                                           & 19,485                                     & 98.46\%                    & 84.34\%                       & 0.9085                       & 0.9717                   & 94.59\%                    & 52.69\%                       & 0.6768                       & 0.9648                   & 63.64\%                    & 41.18\%                       & 0.7669                       & 0.7153                  \\
D2                                           & 12,648                                     & 99.39\%                    & 89.07\%                       & 0.9395                       & 0.9885                   & 92.07\%                    & 52.98\%                       & 0.6726                       & 0.9654                   & 36.36\%                    & 17.65\%                       & 0.5282                       & 0.6398                  \\
D3                                           & 14,686                                     & 97.89\%                    & 84.36\%                       & 0.9062                       & 0.9728                   & 93.25\%                    & 62.08\%                       & 0.7454                       & 0.9688                   & 63.64\%                    & 35.53\%                       & 0.7682                       & 0.8754                  \\
D4                                           & 7,104                                      & 98.90\%                    & 97.83\%                       & 0.9836                       & 0.9732                   & 90.11\%                    & 46.33\%                       & 0.6120                       & 0.9541                   & 62.73\%                    & 17.02\%                       & 0.7569                       & 0.6633                  \\
D5                                           & 37,279                                     & 99.80\%                    & 88.49\%                       & 0.9381                       & 0.9713                   & 93.69\%                    & 56.72\%                       & 0.7066                       & 0.9691                   & 58.92\%                    & 57.14\%                       & 0.7329                       & 0.7543                  \\
D6                                           & 37,383                                     & 98.31\%                    & 93.19\%                       & 0.9568                       & 0.9777                   & 93.23\%                    & 60.49\%                       & 0.7337                       & 0.9689                   & 61.08\%                    & 30.43\%                       & 0.7522                       & 0.7486                  \\
D7                                           & 10,957                                     & 99.15\%                    & 97.48\%                       & 0.9831                       & 0.9893                   & 88.89\%                    & 48.83\%                       & 0.6303                       & 0.9571                   & 36.36\%                    & 23.53\%                       & 0.5270                       & 0.5789                  \\
D8                                           & 3,183                                      & 97.14\%                    & 97.14\%                       & 0.9714                       & 0.9913                   & 82.86\%                    & 49.90\%                       & 0.6229                       & 0.9521                   & 27.27\%                    & 13.04\%                       & 0.4240                       & 0.5145                  \\
D9                                           & 27,820                                     & 99.74\%                    & 85.16\%                       & 0.9188                       & 0.9743                   & 92.51\%                    & 48.77\%                       & 0.6387                       & 0.9660                   & 27.27\%                    & 19.54\%                       & 0.4253                       & 0.6302                  \\
D10                                          & 40,496                                     & 98.48\%                    & 87.80\%                       & 0.9283                       & 0.9770                   & 93.35\%                    & 61.22\%                       & 0.7395                       & 0.9594                   & 45.45\%                    & 27.78\%                       & 0.6168                       & 0.5683                  \\ \midrule
\textbf{Avg.}                                & \textbf{}                                  & \textbf{98.73\%}           & \textbf{90.49\%}              & \textbf{0.9434}              & \textbf{0.9787}          & \textbf{91.46\%}           & \textbf{54.00\%}              & \textbf{0.6778}              & \textbf{0.9626}          & \textbf{48.27\%}           & \textbf{28.28\%}              & \textbf{0.6298}              & \textbf{0.6689}         \\ \bottomrule
\end{tabular}
\end{table*}

Table.~\ref{TAB:Comp:Task1} presents the performance of three models on the task of logic equivalent gates identification. Firstly, our proposed approach outperforms the other two models on all circuits with an average F1-score of $0.9434$ and AUC of $0.9787$, while DeepGate and FGNN only achieve F1-Score $0.6778$ and $0.6298$, and AUC $0.9636$ and $0.6689$, respectively. For instance, in circuit D7, our proposed functionality-aware circuit learning approach exhibits an F1-Score of $0.9831$ and recognizes $99.15\%$ of logic equivalent gate pairs with a precision of $97.48\%$, indicating a low false positive rate. In contrast, DeepGate only achieves an F1-score of $0.6303$, while FGNN fails on most of the pairs. Secondly, although DeepGate has an average recall of $91.46\%$, its precision is only $54.00\%$, indicating a large number of false positive identifications. This is because DeepGate can only find logic equivalent pairs by predicting logic probability, which leads to incorrect identification of gate pairs with similar logic probability. In $80.83\%$ of false positive pairs, the model incorrectly identifies gate pairs with similar logic probability as functionally equivalent. Thirdly, FGNN achieves the lowest performance among the other models with only $0.6689$ AUC and $0.6298$ F1-Score. The poor performance of FGNN is attributed to the weak supervision in the constrastive learning. As FGCN is trained in self-supervised manner, the weak supervision signal derived from perturbing circuit local structures can only guide to distinguish whether the structurally similar circuits have the same function. However, in practical applications, two circuits may have the same function even if their topological structures are extremely different. Therefore, the weak supervision limits the effectiveness of FGNN in identifying logic equivalent gates. 

\begin{table}[!t]
\centering
\caption{Accuracy of Different Models on Functional Similarity Prediction} \label{TAB:Comp:Task2}
\begin{tabular}{@{}ll|lll@{}}
\toprule
Circuit   & \#Gates   & Our              & DeepGate~\cite{li2022deepgate}  & FGNN~\cite{wang2022functionality}  \\ \midrule
D1        & 19,485    & 94.97\%          & 67.00\%          & 68.22\%          \\
D2        & 12,648    & 96.72\%          & 69.64\%          & 86.00\%          \\
D3        & 14,686    & 94.72\%          & 70.68\%          & 69.20\%          \\
D4        & 7,104     & 95.82\%          & 69.93\%          & 70.38\%          \\
D5        & 37,279    & 94.99\%          & 69.41\%          & 76.99\%          \\
D6        & 37,383    & 95.13\%          & 66.76\%          & 80.67\%          \\
D7        & 10,957    & 94.87\%          & 69.39\%          & 82.19\%          \\
D8        & 3,183     & 92.28\%          & 68.26\%          & 71.60\%          \\
D9        & 27,820    & 94.69\%          & 68.89\%          & 75.67\%          \\
D10       & 40,496    & 96.17\%          & 69.05\%          & 80.01\%          \\ \midrule
\textbf{Avg.} & \textbf{} & \textbf{95.04\%} & \textbf{68.90\%} & \textbf{76.09\%} \\ \bottomrule
\end{tabular}
\end{table}

Besides, we list the performance on functional similarity prediction in Table.~\ref{TAB:Comp:Task2}. our approach outperforms the other two on all circuits achieving an average accuracy of $95.04\%$, while the accuracy achieved by DeepGate and FGNN approaches range from $66.76\%$ to $69.93\%$ and from $68.22\%$ to $82.19\%$, respectively. For instance, our approach shows $94.87\%$ accuracy in modeling functional similarity of circuit D7, while the FGNN achieves $82.19\%$ and DeepGate achieves an accuracy of $69.39\%$ on the functional similarity prediction. To summarize, our proposed approach shows better performance than the other circuit learning models~\cite{li2022deepgate, wang2022functionality} on both logic equivalent gates identification and functional similarity prediction. 


\subsection{Effectiveness of Model Design} \label{Sec:Exp:Model}
\subsubsection{PI Encoding Strategy}
To demonstrate the effectiveness of proposed PI encoding (PIE) strategy, we train another model without assigning unique identifications for PIs, which is named as \textit{w/o PIE}. The results are shown in Table.~\ref{TAB:ABS:PIE}, where by disabling the PIE decreased the accuracy of predicting functional similarity from $95.04\%$ to $83.50\%$, resulting in an average reduction of $11.87\%$.

% 这种减少的原因是：正如Sec所述的failure case，失去PIE策略的one-round GNN模型无法建模电路的结构信息。更具体的说，我们使用w/ PIE模型的hs embedding用于重汇聚结构识别任务上的准确率为93.22%，而w/o模型的准确率仅为74.56%。而节点功能收到输入节点功能和输入节点之间的是否存在重汇聚影响，一旦无法准确识别重汇聚结构，也就不可能准确地学习节点功能。
Such reduction can be attributed to the fact that, as demonstrated as the failure case in Section.~\ref{Sec:Exp:Model} and Fig.~\ref{FIG:RC}, the one-round GNN model without the PIE strategy cannot model the structural information of the circuit. More specifically, the accuracy of the reconvergence structure identification task with w/ PIE model is $93.22\%$, while the w/o model only achieve $74.56\%$. The functionality of logic gate is affected by both functionality of fan-in gates and whether there is reconvergence between its fan-in gates. Once the reconvergence structure cannot be accurately identified, node functionality cannot be modeled accurately.

\begin{table}[!t]
\centering
\caption{Accuracy Comparison between w/ PIE and w/o PIE on Functional Similarity Prediction} \label{TAB:ABS:PIE}
\begin{tabular}{@{}l|lll@{}}
\toprule
Circuit       & \textit{w/ PIE } & \textit{w/o PIE} & Reduction \\ \midrule
D1            & 94.97\%          & 80.36\%          & 14.61\%          \\
D2            & 96.72\%          & 87.33\%          & 9.39\%           \\
D3            & 94.72\%          & 89.00\%          & 5.72\%           \\
D4            & 95.82\%          & 81.09\%          & 14.73\%          \\
D5            & 94.99\%          & 86.89\%          & 8.10\%           \\
D6            & 95.13\%          & 83.98\%          & 11.15\%          \\
D7            & 94.87\%          & 83.04\%          & 11.83\%          \\
D8            & 92.28\%          & 73.37\%          & 18.91\%          \\
D9            & 94.69\%          & 84.72\%          & 9.97\%           \\
D10           & 96.17\%          & 81.84\%          & 14.33\%          \\ \midrule
\textbf{Avg.} & \textbf{95.04\%} & \textbf{83.16\%} & \textbf{11.87\%} \\ \bottomrule
\end{tabular}
\end{table}

\subsubsection{Aggregator Function}
We compare the gate-specific aggregator (abbreviated as Our, see Section.~\ref{Sec:Exp:Model}) with the convolutional sum aggregator (abbreviated as Conv\_Sum)~\cite{kipf2016semi} and the aggregators in DAGNN~\cite{thost2021directed} (named as DAGNN). Our aggregator have independent learnable parameters when processing gates with different gate types, while the other two share the same parameters. Besides, we design another settings (10-Round), where the model equips the proposed aggregator but performs $10$ forward and backward message-passing rounds. 

From this table, we make two observations. First, the proposed achieves an average accuracy of $95.04\%$, which is better than the other aggregators, including $94.48\%$ for Conv\_Sum and $90.89\%$ for DAGNN. Furthermore, our aggregator exhibits the highest accuracy on $10$ circuits among all settings. Hence, the gate-specific aggregator is beneficial for functionality-aware learning. Second, despite performing more message-passing operations, the accuracy of our model decreases by $6.96\%$ in the 10-Round setting. We find that the model tends to generate similar embeddings for gates with short spatial distances. This can be explained by the fact that as the number of message-passing rounds increases, the node embeddings become more similar, leading to over-smoothing~\cite{li2018deeper}. 

\begin{table}[!t]
\centering
\caption{Accuracy Comparison with Different Aggregator on Functional Similarity Prediction} \label{TAB:ABS:Aggr}
\begin{tabular}{@{}l|llll@{}}
\toprule
Circuit       & \multicolumn{1}{c}{Our} & \multicolumn{1}{c}{Conv\_Sum} & \multicolumn{1}{c}{DAGNN} & \multicolumn{1}{c}{10-Round} \\ \midrule
D1            & 94.97\%                   & 93.30\%                       & 91.02\%                   & 90.40\%                      \\
D2            & 96.72\%                   & 96.12\%                       & 92.99\%                   & 90.38\%                      \\
D3            & 94.72\%                   & 94.65\%                       & 91.83\%                   & 89.18\%                      \\
D4            & 95.82\%                   & 95.32\%                       & 93.12\%                   & 86.74\%                      \\
D5            & 94.99\%                   & 94.30\%                       & 88.07\%                   & 86.35\%                      \\
D6            & 95.13\%                   & 94.48\%                       & 91.54\%                   & 88.92\%                      \\
D7            & 94.87\%                   & 94.67\%                       & 92.10\%                   & 88.90\%                      \\
D8            & 92.28\%                   & 91.66\%                       & 89.99\%                   & 84.61\%                      \\
D9            & 94.69\%                   & 94.60\%                       & 88.34\%                   & 86.37\%                      \\
D10           & 96.17\%                   & 95.70\%                       & 89.90\%                   & 88.94\%                      \\ \midrule
\textbf{Avg.} & \textbf{95.04\%}          & \textbf{94.48\%}              & \textbf{90.89\%}          & \textbf{88.08\%}             \\ \bottomrule
\end{tabular}
\end{table}

\subsection{Effectiveness of Training Strategies} \label{Sec:Exp:Train}
\subsubsection{Curriculum Learning}
To investigate the effectiveness of our curriculum learning (CL) strategy, we train another model with all loss functions in only one stage, instead of adding the functionality-aware loss function in the second stage. The w/ CL model learn to predict the logic probability and structural correlation in the first stage and learn the more difficult task, which predicts the functionality in the second stage. The results are shown in Table.~\ref{TAB:ABS:CL}, where the model w/ CL achieves an accuracy of $94.80\%$ on average and the model w/o CL achieves only $84.50\%$. 

\begin{table}[!t]
\centering
\caption{Performance Comparison between w/ CL and w/o CL on Functional Similarity Prediction} \label{TAB:ABS:CL}
\begin{tabular}{@{}llll@{}}
\toprule
Circuit       & \textit{w/ CL}   & \textit{w/o CL}  & Reduction        \\ \midrule
D1            & 93\%             & 84\%             & 9\%              \\
D2            & 98\%             & 84\%             & 14\%             \\
D3            & 96\%             & 88\%             & 8\%              \\
D4            & 94\%             & 89\%             & 5\%              \\
D5            & 96\%             & 92\%             & 4\%              \\
D6            & 92\%             & 87\%             & 5\%              \\
D7            & 95\%             & 80\%             & 15\%             \\
D8            & 92\%             & 74\%             & 18\%             \\
D9            & 97\%             & 84\%             & 13\%             \\
D10           & 94\%             & 83\%             & 11\%             \\ \midrule
\textbf{Avg.} & \textbf{94.70\%} & \textbf{84.50\%} & \textbf{10.20\%} \\ \bottomrule
\end{tabular}
\end{table}

% 我们分析出现这种情况的原因如下。在学习节点功能的任务上，对比任意一对逻辑门的开销太大（与电路大小的平方成正比），且probability相同是功能等价的必要条件，我们限定了模型只需要在probability相似的节点对中学习功能相似性。因此，当模型不采用分阶段训练的策略时，这样的数据集就不能有效地监督训练，也就会出现在预测功能任务上表现不佳的情况。正如表格中所示，两种模型之间$L_{prob}$和$L_{rc}$之间相差不大，也就是说他们在预测logic probability和识别重汇聚结构的任务上性能类似，但在学习功能性上表现不佳。
We analyze the reason as follows. The cost of comparing each pair of logic gates in the task of learning functionality is extremely high, which is proportional to the square of the circuit size. We limit the dataset and train the model to learn functional similarity only among pairs with similar logic probability, which is a necessary condition for functional equivalence. Therefore, without the staged CL strategy, be effectively supervised with the simplified dataset, leading to poor performance in learning functionality. As shown in Table.~\ref{TAB:ABS:Loss}, the differences between the two models in the loss values for predicting logic probability ($L_{prob}$) and identifying reconvergence structures ($L_{rc}$) are not significant, indicating that they perform similarly in these two tasks. However, the w/o CL model performs poorly in learning functionality, where the $L_{func}$ is $0.1224$ and $105.93\%$ higher than w/ CL model. 

\begin{table}[!t]
\centering
\caption{Loss Comparison between w/ CL and w/o CL} \label{TAB:ABS:Loss}
\begin{tabular}{@{}llll@{}}
\toprule
           & \textit{w/ CL} & \textit{w/o CL} & Reduction   \\ \midrule
$L_{prob}$ & 0.0207         & 0.0205          & 1.02\%  \\
$L_{rc}$   & 0.1115         & 0.1186          & -6.36\%   \\
$L_{func}$ & 0.0594         & 0.1224          & -105.93\% \\ \bottomrule
\end{tabular}
\end{table}


% 1(Done). No CL, Task 123 
% 2(Run). No CL, Task 3
% 3(Run). CL, S1:Task1, S2:Task3

\section{Downstream Tasks}
In this section, we apply our model to practical EDA tasks: logic synthesis and Boolean satisfiability solving. The logic synthesis tools aim to identify logic equivalent gates as quickly as possible. In Section.~\ref{Sec:Task:Sweep}, our proposed functionality-aware circuit learning model provides guidance to these tools about the logic similarity. Additionally, in Section.~\ref{Sec:Task:SAT}, we apply the learnt functional similarity in SAT solving, where the variables with dissimilar functionality are assigned the same decision value. This approach efficiently shrinks the search space by enabling solvers to encounter more constraints.

\subsection{Logic Synthesis} \label{Sec:Task:Sweep}
This subsection shows the effectiveness of our proposed functionality-aware circuit learning framework in SAT-sweeping~\cite{kuehlmann2002robust}, a common technique of logic synthesis. Fig.~\ref{fig:SATsweep} illustrates the components of a typical ecosystem for SAT-sweeping engine (also called SAT sweeper), where including \emph{equivalence class (EC) manager}, \emph{SAT-sweeping manager}, \emph{simulator} and \emph{SAT solver}. All computations are coordinated by the SAT-sweeping manager~\cite{mishchenko2018integrating}. The SAT sweeper starts by computing candidate ECs using several rounds of initial simulation and storing ECs into EC manager. In the next step, the SAT-sweeping manager selects two gates within an EC and then calls the SAT solver to check whether they are equivalent. If so, the EC manager merges these two gates. Otherwise, SAT solver will return a satisfiable assignment as a counterexample for incremental simulation to refine the candidate ECs.

To the best of our knowledge, most SAT-sweeping managers select EC only based on the circuit structure, without efficient heuristic strategy considering the functionality of candidate gates. We will introduce the functional information into SAT-sweeping manager to further improve efficiency. 

\begin{figure}[!t]
    \centering
    \includegraphics[width=1.0\linewidth]{figs/SATSweeping.pdf}
    \caption{The proposed SAT-sweeping ecosystem.}
    \label{fig:SATsweep}
\end{figure}

\subsubsection{Experiment Settings} 
We combine our functionality-aware circuit learning model into SAT sweeper to guide EC selection. To be specific, the updated manager sorts all candidate equivalence classes by computing the cosine similarity of their embeddings. Unlike traditional SAT sweeper, the equivalence of all candidate ECs are not necessary to validate by one pass. The node pair has a higher similarity, it has the priority of SAT solver call. If equivalent, merge this node pair, otherwise, the generated counterexample is more efficient than traditional SAT sweeper, that is, the efficiency of candidate ECs refinement is better.

Our model is equipped into ABC~\cite{abc} as a plug-in and integrated into the SAT-sweeping engine `\texttt{\&fraig}'~\cite{mishchenko2005fraigs}, which is one of the most efficient and scalable SAT sweeper publicly available at this time. The AIGs derived by merging the resulting equivalent nodes are verified by `\texttt{\&cec}' command in ABC to ensure functional correctness. All experiments are performed on a 2.40 GHz Intel(R) Xeon(R) Silver 4210R CPU with 64GB of main memory. A single core and less than 1GB was used for any test case considered in this subsection. The proposed SAT sweeper (named as \emph{Our}) is compared against the original engine, \emph{\&fraig}.

\subsubsection{Results}

% This subsection shows the effectiveness of the proposed functionality-aware circuit learning framework in SAT-sweeping algorithm. Fig.~\ref{fig:SATsweep} illustrates the components of a typical ecosystem for SAT-sweeping based on functionality-aware circuit learning and the interaction between them. All computations are coordinated by the \emph{SAT-sweeping manager}~\cite{mishchenko2018integrating}. It starts by allocating the components and computing candidate equivalence classes using several rounds of random simulation. In the next step, the \emph{functionality-aware learning} manager sorts all candidate equivalence classes by computing their cosine similarity. For example, if a node has a higher similarity, the SAT solver is called to check whether the node is equivalent to the representative of the class. On the contrary, if the node is nonequivalent, the generated CEs can further refine the candidate equivalence classes.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% The algorithm have been implemented in ABC~\cite{abc} and integrated into the SAT-sweeping engine `\texttt{\&fraig}'. The AIGs derived by merging the resulting equivalent nodes are verified by `\texttt{cec}' command in ABC to ensure functional correctness. All experiments are performed on a 2.40 GHz Intel(R) Xeon(R) Silver 4210R CPU with 64GB of main memory. A single core and less than 1GB was used for any test case considered in this subsection. The proposed SAT sweeper is compared against the similar engine, \emph{\&fraig}. To our knowledge, \emph{\&fraig} is the most efficient and scalable SAT sweeper publicly available at this time. 

We validate the performance of our SAT sweeper with $6$ industrial circuits. As shown in Table~\ref{TAB:SATsweep}, section ``Statistics'' lists the number of PI and PO (PI/PO), logic levels (Lev), internal AND-nodes in the original AIG (And), and internal AND-nodes in the AIG after SAT-sweeping (Result). Section ``SAT calls'' lists the number of satisfiable SAT calls, performed by the solver employed in each engine. The data shows that our proposed engine decreases the number of satisfiable SAT calls, that explains why it has better results, since more resource are used to prove equivalent gates. In addition, section ``Total runtime'' compare the runtimes and the amount of runtimes has been accelerated ``$\texttt{x}$''. Finally, we use the average geometric mean improvement of optimized to initialization ``Geo.'' to measure the efficiency of algorithm. The number of ``SAT calls'' can get an average improvement of 2.95$\times$ (24.3$\times$ maximum). As for ``Total runtime'', this experiment shows that the functionality-aware circuit learning based SAT sweeper outperforms state-of-the-art engines, while reducing the average runtime by 2.00$\times$ ($2.36 \times$ maximum). It is due to the fact that our method by increasing the quality of each SAT solving, reduce the inefficiency and even invalid SAT calls, thus improve the runtime.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[!t]
\centering
\caption{Comparing the number of SAT calls and the runtime of the SAT sweepers} \label{TAB:SATsweep}
\setlength\tabcolsep{2.5pt}
\begin{tabular}{@{}lrrrrrrrrr@{}}
\toprule
\multirow{2}{*}{Circuit} & \multicolumn{4}{c}{Statistics} & \multicolumn{2}{c}{SAT calls}  & \multicolumn{3}{c}{Total runtime (s)} \cr
\cmidrule(l){2-5} \cmidrule(l){6-7} \cmidrule(l){8-10} 
       & PI/PO    & Lev  & And     & Result  & \&fraig  & Our   & \&fraig  & Our    & \texttt{x} \cr \midrule
C1     & 128/128  & 4372 & 57,247  & 29,040  & 13,826   & 570   & 7.46     & 3.15   & 2.36        \cr
C2     & 24/25    & 225  & 5,416   & 5,353   & 100      & 74    & 5.43     & 3.11   & 1.74        \cr
C3     & 22/1     & 29   & 703     & 0       & 4        & 1     & 19.07    & 9.10   & 2.09        \cr
C4     & 114/1    & 91   & 19,354  & 0       & 20       & 12    & 6.49     & 4.04   & 1.61        \cr
C5     & 126/1    & 83   & 20,971  & 0       & 6        & 4     & 0.48     & 0.21   & 2.28        \cr
C6     & 96/1     & 79   & 14,389  & 0       & 10       & 5     & 0.30     & 0.15   & 2.00        \cr \midrule
{\bf Geo.} &      &      &         &         &          & {\bf 2.95} &     & {\bf 2.00}   &          \cr
\bottomrule
\end{tabular}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Boolean Satisfiability Solving} \label{Sec:Task:SAT}
% 传统方法怎么做，我们能帮助什么
Boolean satisfiability solving (or SAT solving), a long-standing and fundamental NP-complete problem in many areas, has attracted significant research interest in recent years, which results in the development of many efficient SAT solvers.
These SAT solvers are usually designed to incorporate better heuristics that can either speed up the Boolean Constraint Propagation (BCP) process or help find a better decision ordering.
In this subsection, we demonstrate how the learnt representations can be utilized to enforce a more efficient decision ordering for solving circuit-based SAT instances, which in turn speeds up current SAT solvers.
And our method is dubbed functionality-aware decision ordering.
Specifically, if two circuit signals have similar representations (and therefore similar functionality), their corresponding variables should be grouped together in the search process and assigned opposite values. 
Given the variable set $\mathcal{S}$, when the current variable $s$ is assigned a value $v$ by BCP, we identify all unassigned variables in $\mathcal{S}$ whose representations are similar to $s$ and assign the value $\Bar{v}$ to them. 
To improve the efficiency of our method, we introduce an indicator function $I(\cdot)$ to track whether one variable has been used in functionality-aware decision making. 
And we only consider variables whose indicator functions return a false value.
The details of our method are summarized in Algorithm \ref{Boolean-Satisfiability-Solving}. 

Assigning opposite values to functionality-similar variables is more likely to cause conflicts during the solving process. As a result, learned clauses can be acquired more effectively, which, in turn, accelerates the solving process. Besides, 


\begin{algorithm}[htbp]
    \caption{Functionality-Aware Decision Ordering}
    \label{Boolean-Satisfiability-Solving}
    \textbf{INPUT:} Current variable $s$ just being assigned a value $v$ by BCP; Set of variables $\mathcal{S}$; Function $R(\cdot)$ to retrieve the learnt representation of one variable; Function $V(\cdot)$ to get the assigned value of one variable; Function $\text{sim}(\cdot,\cdot)$ to calculate the similarity of representations of two variables; Indicator $I(\cdot)$ to show whether one variable has been used before; Threshold $\delta$ \newline
    \textbf{OUTPUT:} Variables with similar representations as $s$ and their value assignments
    \begin{algorithmic}[1]
    \FOR{$s^{\prime}$ in $\mathcal{S}$}
    \IF{$s^{\prime} \neq s$ and $V(s^{\prime}) = \text{None}$ and $I(s^{\prime}) = \text{false}$} 
    \IF{$\text{sim}(R(s^{\prime}), R(s)) > \delta$}
    \STATE $V(s^{\prime}) = \Bar{v}$
    \STATE $I(s^{\prime}) = \text{true}$
    \ENDIF
    \ENDIF
    \ENDFOR
    \end{algorithmic}
\end{algorithm}


\subsubsection{Experiment Settings}
% 我们的model怎么加进去（需要注意一定要说明我们是plug-in，不需要改很多代码）
% 画一个algorithm
To evaluate the effectiveness of the learnt representations in accelerating the downstream SAT solving, we adopt the SAT solver, CaDiCaL (\textcolor{red}{cite}), and (\textcolor{red}{test cases}), which are transformed into the Conjunctive Normal Form (CNF) format.


\subsubsection{Results}
\begin{table}[!t]
\centering
\renewcommand\tabcolsep{5.0pt}
\caption{Comparing the Runtime between Baseline and Our Solvers} \label{TAB:SATSolving}
\begin{tabular}{@{}ll|l|lll|l@{}}
\toprule
\multirow{2}{*}{Instance} & \multirow{2}{*}{Size} & \multirow{2}{*}{Baseline(s)}        & \multicolumn{3}{c|}{Our(s)}      & \multirow{2}{*}{Reduction} \\
                          &                       &        & Model     & Solver    & Overall         &                            \\ \midrule
I3                        & 17,495                & 88.01           & 1.77      & 30.25     & 32.02           & 63.62\%                    \\
I1                        & 21,952                & 29.36           & 2.85      & 6.01      & 8.86            & 69.82\%                    \\
I2                        & 23,810                & 61.24           & 3.25      & 32.88     & 36.13           & 41.00\%                    \\
I5                        & 27,606                & 158.04          & 4.36      & 137.77    & 142.13          & 10.07\%                    \\
I4                        & 28,672                & 89.89           & 4.78      & 70.95     & 75.73           & 15.75\%                    \\
I6                        & 34,654                & 934.00          & 6.12      & 890.71    & 896.83          & 3.98\%                     \\ \midrule
\textbf{Avg.}             & \textbf{}             & \textbf{226.76} & \textbf{} & \textbf{} & \textbf{198.62} & \textbf{12.41\%}           \\ \bottomrule
\end{tabular}
\end{table}

